Towards an Objective Metric for the Performance of Exact Triangle Count

The performance of graph algorithms is often measured in terms of the number of traversed edges per second (TEPS). However, this performance metric is inadequate for a graph operation such as exact triangle counting. In triangle counting, execution times on graphs with a similar number of edges can be distinctly different as demonstrated by results from the past Graph Challenge entries. We discuss the need for an objective performance metric for graph operations and the desired characteristics of such a metric such that it more accurately captures the interactions between the amount of work performed and the capabilities of the hardware on which the code is executed. Using exact triangle counting as an example, we derive a metric that captures how certain techniques employed in many implementations improve performance. We demonstrate that our proposed metric can be used to evaluate and compare multiple approaches for triangle counting, using a SIMD approach as a case study against a scalar baseline.

==> TC_Perf cam ready plus ieee copyright/characteristics.tex <==
%I

In this section, we describe properties which we consider desirable in an objective performance metric for hardware-software co-design. We illustrate these properties using dense matrix-matrix multiplication where the use of number of floating point operations per second (FLOPS/s) is a well-established performance metric for dense linear algebra.

%The following properties are proposed to be desirable for a performance metric:
%\begin{enumerate}
% [scott: alternative title: "Indicative of the expected amount of work performed"]
% \subsection{Reflects the Expected Amount of Work}
\subsection{Indicative of the Expected Amount of Work Performed}
    
    A performance metric needs to measure the expected amount of useful work performed as increasing the amount of work necessarily increases the execution time. By work, we mean the basic unit of computation (and data movement) that is \emph{necessary to compute the desired result using a generally accepted algorithm}. It is necessary to note that the expected amount of work is not the minimum amount of work that could be performed. %As we elaborate in Subsection~\ref{subsec:innovations}, algorithmic improvements to reduce the amount of work should be reflected in a higher or better score by virtue that less time is required to compute the desired result.
    
    To illustrate this, consider multiplying two matrices of sizes $m \times k $ and $k \times n$. The quantity of work (measured in floating point operations) is approximately $2mnk$ using the traditional triply-nested loop algorithm. Algorithmic innovations such as Strassen~\cite{STRASSEN1969} reduce the expected amount of work, resulting in a faster execution time and thus a higher FLOPS/s when using $2mnk$ floating point operations as the expected amount of work. This metric can potentially report performance above the theoretical peak of the hardware~\cite{jianyuStrassen} because the expected amount of work exceeds that of the actual work.
    
    %\item {\em Measurement of hardware capabilities.}
\subsection{Measures Hardware Capabilities}
    The performance metric has to be sufficiently low-level to expose hardware capabilities related to the work being performed. %Ideally, the metric should be tied to the hardware capabilities of a given computing platform, where 
    Hardware with more capability for computing the basic work unit should yield a correspondingly increased score using the metric. When normalized to the theoretical capability of the available hardware, the performance metric should also indicate how well the available hardware is being utilized.
    
    %Returning to the matrix matrix multiplication example, the fundamental work units are the floating point operations. 
    
    Increased hardware capabilities such as the introduction of the fused-multiply-accumulate unit (FMA) unit and Single Instruction Multiple Data (SIMD) instruction set extensions can be objectively quantified using FLOPS/s as these hardware capabilities allow more floating point operations to be computed per unit time. Comparing attained FLOPS/s as a function of percentage of theoretical peak hardware capability allows for introspection on implementations to determine if more can be done to achieve better performance.
    
    %Performance comparison between different platforms with different capabilities can easily be normalized by the number of hardware features such as nodes, cores, functional units, and frequency.
    %relates rather directly to an operation performed by hardware. In this case, floating point adds and multiplies are two different operations, but in recent hardwares they are a single fused operation.
    
\subsection{Captures Implementation Innovations}
\label{subsec:innovations}
%    \item {\em Reflection of implementation innovation.} 
    Implementation innovations, such as tiling and data layout changes, increase performance through improved data access while maintaining the amount of work that is performed.  A performance metric should reflect these innovations with a better score despite having no change in both the hardware or the expected amount of work.
    %While reflecting the expected work of some generally-accepted baseline, the metric should also credit useful algorithmic and implementation innovations with a better score. These innovations include but are not limited to data preprocessing and layout, clever algorithms to reduce the number of actual operations performed, and approaches to parallelism.
    
    A high performance matrix matrix multiplication is often implemented as multiple nested loops that partition a matrix into submatrices through loop tiling/blocking~\cite{goto_anatomy_2008,BLIS1}. In addition, input matrices are repacked in order to ensure that 1) data is brought into the appropriate level of caches and 2) data is repacked such that accesses can be performed with unit stride~\cite{ greghenry}. These implementation choices maintain the same amount of (useful) work, but increase the performance due to better data access. These benefits are demonstrated via a higher FLOPS/s score.
    
    %The number of operations that the metric represents can be computed and know ahead of time, simply by examining the input parameters of the problem.
%\end{enumerate}


%For example, general matrix multiply at its core performs floating point multiplies and additions, with a know number of such operations that must be performed for a specific input size.
%The operations being performed also have a known performance peak in hardware terms: the number of pipelined SIMD fused-multiply-accumulates (FMAs), for example. Hence, FLOPs represent a metric that relates the fixed number of operations performed in DGEMM to the hardware that performs them.


 \subsection{Application to Graph Algorithms}
 While we have identified the desirable properties of a performance metric, %there are a number of issues that make it less obvious to identify a metric for a graph algorithm that satisfy the desired properties.
 the vertices of a graph can be relabeled and reordered without changing the structure of the graph. Moreover, the adjacency matrix of the different isomorphic graphs often exhibit different structures that may change the amount of work that needs to be computed. As a convention, we take the original unsorted graph as the canonical graph from which the expected amount of work is computed.  

%Thus, the performance of an algorithm on a re-ordered graph should be measured based on the \textit{effective} number of match checks performed over the runtime, rather than the \textit{absolute} number of match checks for that particular version of the input. 
% The potential benefit of the reordering can still be studied from absolute numbers of match checks, while the implementations' runtimes can be evaluated based on the effective work that each performs.


%The primary goal of this paper is to find a metric that addresses these three desirable properties for a performance metric. 
%Edges per Second is not such a metric: as we will show, it does not reflect the amount of work in triangle counting; it does not directly relate to hardware properties relevant to triangle counting; and innovations of implementation, such as sorting as a preprocessing step, are not reflected.
% The choice of a metric that connects algorithmic operations to hardware operations is crucial.
%An objective performance metric enables both designers of algorithms and software as well as hardware architects to understand how much hardware potential is realized in an implementation and to fairly compare implementations across inputs.

==> TC_Perf cam ready plus ieee copyright/conclusion.tex <==
In this work, we proposed the use of match checks and match checks per cycle as a performance metric for exact triangle counting. This is motivated by the need for a metric that explains the performance of triangle counting implementations in terms of the amount of work and the hardware capabilities of the system.

We demonstrated that the metric represents the amount of work that has to be performed in triangle counting. The metric also provides new insights into commonly-employed techniques found in many triangle counting implementations such as sort-based relabeling. While we have focused on only sequential implementations, we believe that extending the metric to represent parallel implementations should be straight-forward. 

The observant reader may note that match checks and the number of actually traversed edges in the graph are very similar in numeric value. 
In fact, the actual number of edges traversed equals the number of match checks plus the number of triangles in the graph.
The case we make in this work is not that match checks are better than counting the number of truly traversed edges, but that edges-per-second as used in many recent works is not appropriate and some hardware-focused metric like match checks is needed for hardware-software co-design.

More generally, we believe that the approach we took to identify the proposed metric can be replicated for different (classes of) graph algorithms to identify objective metrics. Having better metrics would provide greater insights into the amount of work to be performed and the hardware capabilities that are required. These insights could lead to faster and more efficient software implementations, and could also suggest hardware features needed by graph algorithms. 

Identified metrics for one graph algorithm could potentially apply to other graph algorithms. For example, the set intersection kernel in triangle counting is similar to a sparse dot product. This suggests that other graph algorithms and sparse linear algebraic workloads may benefit from similar metrics for performance evaluation. We will pursue these directions in future work.

\section*{Acknowledgement}
This material is based upon work funded and supported by the Department of Defense under Contract No. FA8702-15-D-0002 with Carnegie Mellon University for the operation of the Software Engineering Institute, a federally funded research and development center [DM20-0657].

Mark Blanco is supported by the National Science Foundation Graduate Research Fellowship Program under Grant No. DGE 1745016. Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.
%In summary, this work seeks to address the limitations of using Edges Per Second as a performance metric for exact triangle counting (TC).
%The vast majority of works on triangle counting have used this figure to indicate performance, when in fact it offers little to no insight over looking at raw runtime. 

%As an alternative, we proposed a basic metric based on examination of a naive scalar kernel for TC: Match Checks per Second (MCs).
%We motivated the metric by its ability to better describe the amount of work performed in a triangle counting implementation based on identifying matching pairs of vertex IDs that complete a found triangle.
%{\color{blue}{Pearce et al. make explicit reference to ``wedge-checks (triangle closure checks),'' in \cite{pearce_one_2019}, neither this work nor any other we are aware make a strong case to adopt such a metric for general performance analysis of triangle counting implementations.}}

%By using graph reordering, a common preprocessing step, we illustrated the descriptive value of the metric: in the oregon1\_010519 of the GraphChallenge collection the match checks to be performed decreased by 97 percent, leading to a 19.9x speedup for the same scalar implementation;
%when sorting in the reverse order increased the number of checks performed in p2p-Gnutella09 by 30 percent, processing the graph took 4.2 times longer.
%Using a work-inefficient SIMD implementation as an example, we showed that the metric can apply to more complex approaches by way of measuring performance in terms of Effective Match Checks per Second (EMCs), both in a microbenchmark setting and on real-world graphs.

%Effective Match Checks per Second as a metric is intended to be a useful tool in focusing researchers' reasoning about exact triangle counting implementations and how those implementations perform on various graphs and hardware.
%Using EMCs as a starting point, we hope to bring the community's understanding of TC one step closer to being able to reason about implementation performance in terms of hardware performance peaks.

%Finally, we note that the kernel identified at the heart of triangle count is not very different from a sparse dot product. 
%Hence, other graph algorithms and sparse linear algebraic workloads may benefit from similar metrics for performance evaluation. 
%This is but one possible direction for future work.

==> TC_Perf cam ready plus ieee copyright/conclusion_draft.tex <==
In summary, this work seeks to address the limitations of using Edges Per Second as a performance metric for Exact Triangle Counting (TC).
As an alternative, we proposed a basic metric based on examination of a naive scalar kernel for TC: Matche Checks per Second (MCs).
We motivated the metric by its ability to better describe the amount of work performed in a triangle counting implementation based on identifying matching pairs of vertex IDs that complete a found triangle.
By using graph reordering, a common preprocessing step, we illustrated the descriptive value of the metric:
in the oregon1\_010519 of the GraphChallenge collection the match checks to be performed decreased by 97 percent, leading to a 19.9x speedup for the same scalar implementation;
when sorting in the reverse order increased the number of checks performed in p2p-Gnutella09 by 30 percent, processing the graph took 4.2 times longer.
Using a work-inefficient SIMD implementation as an example, we showed that the metric can apply to more complex approaches by way of measuring performance in terms of Effective Match Checks per Second (EMCs).

Effective Match Checks per Second as a metric is intended to be a useful tool in focusing researchers' reasoning about Exact Triangle Counting implementations and how those implementations perform on various graphs and hardware.
Using EMCs as a starting point, we hope to bring the community's understanding of TC one step closer to being able to reason about implementation performance in terms of hardware performance peaks.

==> TC_Perf cam ready plus ieee copyright/evaluation_simd_scalar.tex <==
%\subsection{Matches Reflecting Implementation Innovation}
%In this final subsection, we introduce one more variant of the 8x8 SIMD 
%set intersection kernel.
%This version of the kernel includes the blue lines of code in Algorithm~\ref{alg:simd_8x8_inter}.
%The additional lines check that the two input sections of each set overlap based on the first and last values in each. 
%If they do not, the loop will continue without executing any of the SIMD comparisons. We call this version of the SIMD kernel `skip-ahead SIMD.'
%We use the skip-ahead SIMD kernel as an example of an implementation innovation over the 8x8 SIMD kernel, where better performance should be reflected in effective match-check rate.
% As we discuss in the next section, the concept of \textit{effective} matches per second or per cycle is also useful for comparing 
% implementations that perform a very different amount of work in hardware but are nonetheless usually faster in terms of runtime.

%\begin{figure}
%    \centering
    % \includegraphics[width=\linewidth]{figures/haswell_effective_cmps_per_cycle.pdf}
%    \includegraphics[width=\linewidth]{figures/Evaluation of Implementation Innovation for 3 Architectures.pdf}
%    \caption{Effective match checks per cycle for Skylake-X (SKX), Kaby Lake (KBL), and Zen 2 CPU architectures for scalar, 8x8 SIMD, and 8x8 SIMD `skip-ahead' set intersection kernels.}
%    \label{fig:ubench_simd_vs_simd}
%    \vspace{-5mm}
%\end{figure}

%Fig.~\ref{fig:ubench_simd_vs_simd} shows the effective match checks per cycle across all of the test patterns, for the scalar implementation as well as the two SIMD implementations.
%Across the three architectures, the improvements of each successive variant over the previous approaches are clearly visible in terms of match checks per cycle.
%Thus, the effective match check rate as a metric of performance clearly reflects the implementation innovation present in the kernel variants.

%In this section, we demonstrated that match checks are a meaningful and fair measure of work for triangle counting. 
%Through micro-benchmarks on set intersection, the core operation in triangle counting, we further demonstrated that the effective match check rate can be used to study how well the hardware is utilized and to compare levels of performance between multiple implementations.
% \subsection{SIMD Set Intersection}


% In this section we describe a SIMD-based set intersection kernel. 

% In SIMD, it is possible to load and compare multiple values at the same time.
% If one SIMD register contains contiguous values from one neighborhood, and the other register contains a single
% value broadcast from the other neighborhood, the SIMD compare operation accomplishes match checks between that one element and all elements in the first register.
% It is possible for no matches to be found, or a single match to be found. 
% In some cases, the match that succeeds may be between the broadcast value and some value in the middle of the first SIMD register. 
% In this case, the match checks that were tested for later values in the first register are \textit{wasteful} - they would not have occurred in the scalar implementation processing the same neighborhoods. 
% This concept of wasteful match checks is a direct result of using SIMD to unroll the scalar loop and speculatively perform a set of match tests.








==> TC_Perf cam ready plus ieee copyright/hardware_peak.tex <==
\subsection{Matches Reflected in Hardware Capability}

\begin{algorithm}[tb]
\DontPrintSemicolon
% \SetAlgoLined
\smaller
\KwIn{a1 and a2 initially give the start addresses of each set. a1\_nd and a2\_nd are the addresses just after the end of each set.}
\KwOut{$\Delta$ is the number of matches among both sets.}
\BlankLine
$\Delta$ $\leftarrow 0$ \\
\While{a1 $<$ a1\_nd $\land$ a2 $<$ a2\_nd} {
  a1\_max $\leftarrow$ a1[7]\\
  a2\_max $\leftarrow$ a2[7]\\
  %{\color{blue}
  \tcp*[l]{Early termination checks}
  a1\_min $\leftarrow$ a1[0]\\
  a2\_min $\leftarrow$ a2[0]\\
  \If{a1\_max $<$ a2\_min}{a1 $\leftarrow$ a1 + 8; continue}
  \If{a2\_max $<$ a1\_min}{a2 $\leftarrow$ a2 + 8; continue}
  %}
  vector\_1[0:7] $\leftarrow$ a1[0:7] \\
  \tcp*[l]{packed load}
  vector\_2\_1[0:7] $\leftarrow$ a2[0] \\
  \tcp*[l]{broadcast}
  \tcp*[l]{Omitted: similar broadcasts for a2[1] through a2[7]...}
 
  cmp\_mask\_1 $\leftarrow$ cmp\_eq(vector\_1, vector\_2\_1)\\
  cmp\_mask\_2 $\leftarrow$ cmp\_eq(vector\_1, vector\_2\_2)\\
  cmp\_mask\_3 $\leftarrow$ cmp\_eq(vector\_1, vector\_2\_3)\\
  cmp\_mask\_4 $\leftarrow$ cmp\_eq(vector\_1, vector\_2\_4)\\
  cmp\_mask\_5 $\leftarrow$ cmp\_eq(vector\_1, vector\_2\_5)\\
  cmp\_mask\_6 $\leftarrow$ cmp\_eq(vector\_1, vector\_2\_6)\\
  cmp\_mask\_7 $\leftarrow$ cmp\_eq(vector\_1, vector\_2\_7)\\
  cmp\_mask\_8 $\leftarrow$ cmp\_eq(vector\_1, vector\_2\_8)\\
  %\tcp*[l]{similar compare operations for cmp\_mask\_2 - cmp\_mask\_7...}
 
  \tcp*[l]{Omitted: logically or all cmp\_masks together into and\_mask...} 
  $\Delta \leftarrow \Delta$ + popcount(and\_mask) \\ 
  \If{a1\_max $\leq$ a2\_max}{a1 $\leftarrow$ a1 + 8}
  \If{a2\_max $\leq$ a1\_max}{a2 $\leftarrow$ a2 + 8}
  }
  \Return{$delta$}
  \caption{SIMD 8x8 set intersection kernel. Leftover set elements go to the scalar kernel.}
  \label{alg:simd_8x8_inter}
\end{algorithm}

Here we introduce a case study of using match checks to evaluate an alternate approach (SIMD) against a baseline (merge-based scalar) with a focus on hardware-software co-design.
Single-instruction multiple-data (SIMD) hardware is commonly used in regular applications due to the higher throughput it affords.
Use of SIMD in graphs is less common as graph algorithms (inclusive of triangle counting) are considered irregular.
Using match checks, we showcase that SIMD is measurably faster than the scalar approach owing to performing more \textsl{effective} match checks per cycle. 

Recall that match checks can be used as a proxy for the number of times a compare (\texttt{CMP}) instruction is required. The use of SIMD compare instructions (e.g. \texttt{VPCMPEQ}) can increase the number of comparisons that are performed, thus increasing the overall throughput. 

\begin{figure}
    \centering
    \includegraphics[width=0.87\linewidth]{figures/match_patterns_CROPPED.png}
    \caption{Different distributions of vertex IDs results in different number of match checks. Arrows show the match checks that will be performed by Algorithm 1. The interleaved pattern has the largest number of match checks (15) between two neighborhoods of size 8 each. 
    %Top left to bottom right: interleaved, all-matching, disjoint, and even-vs-even-squares. 
    }
    \label{fig:match_patterns}
    \vspace{-5mm}
\end{figure}

We implemented multiple SIMD set intersection kernels, one of which is shown in Algorithm~\ref{alg:simd_8x8_inter}. This kernel compares eight vertices from each neighborhood against each other. This effectively computes 64 match checks within the kernel. 
However, notice that the number of SIMD match checks corresponding to match checks which the scalar implementation would have performed depends on the distribution of vertex IDs in each vector.
The impact of the different distribution of vertex IDs is illustrated in Fig.~\ref{fig:match_patterns}.
In our analysis, we therefore consider \textit{effective} match checks, where performance of the SIMD approach is measured based on the number of effective match checks it performs relative to the scalar baseline.
The remaining match checks performed in the SIMD approach are considered wasted work.

%triangle counting is irregular due to the data-dependent control flow of the set intersections as in Algorithm~\ref{alg:scalar_inter}.
%A SIMD kernel for set intersection approaches this problem by effectively unrolling the scalar loop and speculatively executing match checks that may not need to be done.
%Algorithm~\ref{alg:simd_8x8_inter} illustrates the SIMD approach wherein each iteration of the loop body core (lines 13 through 28)
%tests all match checks for eight elements from the first neighborhood against four elements from the second. 
%For this subsection, we ignore the lines highlighted blue (5-10).
% The SIMD kernel is in essence a reduced outer product of $8 \times 4$ elements. 
%Note that at most four match checks can possibly succeed, and some number of the remaining match tests performed would
%never have been performed in the scalar approach.

%In spite of this inefficiency, we show through microbenchmarks that SIMD often achieves a higher effective match test rate (i.e. match checks-per-cycle) than the scalar implementation for a number of set intersection input patterns shown in Figure~\ref{fig:match_patterns}.
%The cases are all-matching, interleaved-values, disjoint-values, reversed-disjoint-values, and evens-vs-even-squares
%With the exception of reversed-disjoint-values these are pictured in Fig.~\ref{fig:match_patterns}.

%Examining two different implementations of triangle counting that use different hardware capabilities allows us to apply effective match checks {\color{red}{What is the effective match check here?}} as a metric in evaluating attained performance as a function of hardware capabilities.
%We use effective match checks in order to relate the work of checking matches to the operations executed by hardware.

The performance of triangle count using the scalar and SIMD versions of the set-intersection kernels, in match checks-per-cycle, is reported in Fig.~\ref{fig:overall} for the following systems:
\begin{itemize}
    \item[--] Intel Xeon E5-2667 CPU (Haswell)
    \item[--] Intel i7-7700K CPU (Kaby Lake)
    \item[--] Intel Xeon Platinum 8153 CPU (Skylake-X)
    % \item[--] an AMD Ryzen 5 3600X CPU (Zen 2)
\end{itemize}

Sequential performance numbers are shown for all graphs, which are relabeled in decreasing vertex degree order. Sorting time is NOT included in the overall execution time. The graphs in each plots are ordered by increasing graph size (size in memory).

The utility of SIMD set intersection is mixed on the sorted graphs. For smaller graphs, scalar outperforms SIMD. This is likely due to smaller neighborhoods in small graphs reducing opportunities to apply the SIMD kernels. 
The added logic for switching between multiple kernels and the wasted work in the SIMD approach are potential reasons for diminished performance of the SIMD implementation. 
Additionally, the standard deviation of the lower-neighborhood size for most graphs is reduced after sorting, so there are fewer large neighborhoods that SIMD can process.
For larger graphs, in spite of the wasted work, SIMD is often faster than the scalar implementation.
This implementation innovation is reflected in the effective match checks per cycle shown in Fig.~\ref{fig:overall}, particularly for larger graphs.
 

%For the scalar merge-based implementations, each match check approximately corresponds to three compare operations: one for the actual comparison, and possibly up to two more to check the limits of the set array pointers.
%Based on the Intel Programmer's Guide \cite{noauthor_intel_2020} and instruction timings for the three architectures~\cite{fog_lists_2018}, each CPU is capable of four independent compare operations per cycle.
%Therefore, we might expect at best a peak of $\frac{4}{3} = 1.25$ match checks per cycle for the scalar approach.

\begin{figure*}
\begin{tabular}{c}
\includegraphics[width=1\textwidth]{figures/full_tc_reruns/hsw-chart.pdf}
       \\
\includegraphics[width=1\textwidth]{figures/full_tc_reruns/kbl-chart.pdf}
     \\
\includegraphics[width=1\textwidth]{figures/full_tc_reruns/skx-chart.pdf}
     \\
\end{tabular}
\caption{Scalar and SIMD triangle count performance, in match checks-per-second, for a variety of graphs from the SNAP dataset on Top) Haswell, Middle) Kabylake, and Bottom) Skylake-X architectures. Use of of SIMD instructions results in higher attained performance for graphs with larger neighborhoods. }
\label{fig:overall}
\end{figure*}
%\begin{figure}
%    \centering
    % \includegraphics[width=\linewidth]{figures/haswell_effective_cmps_per_cycle.pdf}
    % \includegraphics[width=\linewidth]{figures/skylakeX_effective_cmps_per_cycle.pdf}
    % \includegraphics[width=\linewidth]{figures/kabylake_effective_cmps_per_cycle.pdf}
    % \includegraphics[width=\linewidth]{figures/zen_2_effective_cmps_per_cycle.pdf}
%    \includegraphics[width=\linewidth]{figures/Set Intersection Microbenchmark Average Performance.pdf}
    %\caption{Average effective match checks per cycle for scalar and 8x8 SIMD set intersection kernels on Skylake-X, Kaby Lake, and Zen 2. Approximate peak in match checks per cycle enables estimating how much hardware performance is realized.}
%    \label{fig:ubench_2}
%    \vspace{-5mm}
%\end{figure}

%For the SIMD approach, we estimate a peak of performance by relating the peak SIMD compare throughput to the expected number of effective match checks per loop body in an 8x8-way SIMD comparison kernel.
%Each SIMD compare operation performs eight match checks for pairs of 32-bit integers but not all of these match checks may be performed in the scalar version.
%In the 8x8 kernel, at best 15 of the 64 total checked matches can yield useful match checks (derived from the interleaved case in Fig.~\ref{fig:match_patterns}).
%The peak per-cycle SIMD-compare throughput for the Intel systems is 2 per cycle, and for Zen 2 it is 1 per cycle.
%We estimate the peak in match checks per cycle as
%$$MATCH_{PEAK} = CMP_{PEAK} \times V_{LEN} \times E_{PEAK}$$
%Where $CMP_{PEAK}$ is the hardware peak for SIMD compares, $V_{LEN}$ is 8 for each AVX2 SIMD vector, and $E_{PEAK}$ is $\frac{15}{64}$.
%From this, Zen 2 can reach at most 1.875 effective matches per cycle, while Skylake-X and Kaby Lake are limited to 3.75 effective matches per cycle.
%Fig.~\ref{fig:ubench_2} shows performance across the test patterns for the three architectures. Neither of the kernels reach over 50\% of peak for either kernel, indicating other performance limitations and possibly that better performance may be obtained.

%This sort of peak estimate using match checks is preliminary, but showcases that match checks enable quantitative reasoning about the level of performance achieved in an implementation out of what is possible.

==> TC_Perf cam ready plus ieee copyright/intro.tex <==
It is widely accepted that software-hardware co-design is required for attaining high performance implementations. 
Therefore, any performance metric used in design and evaluation of an implementation must have properties that bridge the gap between a platform's capabilities and the operations inherent to the problem. 

For many graph algorithms, traversed edges per second (TEPS) is a widely used figure of merit. 
While TEPS suggests that performance is related to the number of edges
that are traversed (read/written during the course of the computation) over time, 
a more common (mis)use of the metric is simply the number of edges in the graph divided by execution time. In many works on triangle counting specifically, the metric used is the simpler definition~\cite{wolf_fast_2017, hu_trix:_2017, samsi_static_2017, mailthody_collaborative_2018, bisson_static_2017}.
From here, we refer to this common usage as edges-per-second.

% Comment Mark: removed to save space, since this paragraph's gist is repeated later anyway.
% {\color{blue}
% While this metric allows one to compare the performance of different implementations running on the same platform and on the same input graph, 
% such a metric is not sufficiently detailed to evaluate why one combination of algorithm, implementation, and hardware platform achieves better performance than a different implementation, either on the same or on a different platform.
% }
%1) which optimizations are important for a given graph operation, 2) which hardware components are essential for improving the performance graph algorithms, and 3) if performance opportunities are not being exploited on current hardware.
%Triangle counting is no exception - since introduction into the GraphChallenge competition, 

To illustrate the inadequacy of the edges-per-second metric for a graph operation such as exact triangle count, consider the plot in Fig.~\ref{fig:motivation} wherein we report the metric performance obtained from a sequential implementation of triangle count for several graphs from the Graph Challenge Dataset~\cite{samsi_static_2017, snapnets}. 
For each graph, we report performance numbers for three different ways in which the vertices have been labeled and sorted.  
Notice that despite having the same number of edges, vertices, and triangles, the performance numbers attained for each graph vary dramatically even when using the edges-per-second metric. 
In essence, the metric is as informative as raw execution time. 
It provides little insight into the software innovation or the hardware capabilities that contribute to the attained performance.

%Triangle Counting is commonly used as benchmark graph application, present both in the Graph Analytics Benchmark initiative and as an established GraphChallenge problem \cite{beamer_gap_2017, samsi_static_2017}. 
%Since the introduction of the GraphChallenge, performance for triangle counting (TC) has increased manyfold~\cite{samsi_static_2017, sam_static_2019}. 
%The sources of these improvements are many: better algorithmic efficiency, higher utilization of parallelism through fine-grained parallelism and load-balancing; access to increasing amounts of parallelism through use of GPUs, multiple CPU nodes, and heterogeneous computing simultaneously processing on both CPU and GPU cores; and strategies for graph partitioning and sorting \cite{lee_family_2017, voegele_parallel_2017, bisson_static_2017, bisson_update_2018, balaji_when_2018}.
%Throughout this, triangle counting has lacked a meaningful metric that relates to the work being performed and can be used to compare implementations across platforms, graphs, and implementations.
% Instead, performance is reported interms of Edges Per Second or some similar variant, even though this figure of merit has little to do with the work being performed at the core of TC.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/graph_reordering_and_time_plot.pdf}
    \caption{The inadequacy of the edges-per-second performance metric is demonstrated by how the metric varies widely for the each graph that has been sorted in different order, while still retaining the same number of edges, vertices and triangles.}
    \label{fig:motivation}
    \vspace{-7mm}
\end{figure}

Samsi et. al.~\cite{graphchallenge_analysis1,graphchallenge_analysis2} use edges-per-second and the metric:
\[
T_{tri} = \left(\frac{N_e}{N_1}\right)^\beta,
\]
where $T_{tri}$, $N_e$, and $N_1$ correspond to the execution time, number of edges in a graph, and number of edges processed in one second. In this metric, $\beta$ is a value (smaller is better) representing  technology advancement that arises from implementation, algorithmic, or hardware improvements.
This metric, however, does not explain the difference in execution times seen in Fig.~\ref{fig:motivation}. In addition, it is unclear how this metric can be used to account for the different aspects of technology improvements such as hardware differences and algorithmic improvements.

In this paper, we propose two performance metrics (match checks, and match checks per unit time) that we believe are more objective than edges-per-second. These metrics more accurately describe the performance of triangle counting attained in Fig.~\ref{fig:motivation}, and better capture the relationship between execution time and the expected amount of work that has to be performed. In addition, the proposed metrics expose the relationship between the amount of work and the hardware capabilities required to perform the required work, which in turn provides newer insights into commonly used techniques employed in many triangle counting implementations.

%describes the amount of work done in counting triangles in a way that relates to a system's hardware capabilities.
%The metric we seek to identify is in the spirit of hardware performance metrics, such as floating point operations per second (FLOPs), integer operations per second (IOPs), and data transferred in some period of time (bytes per second).
%Our primary motivation for identifying a performance metric that reflects the work in Triangle Counting is to offer a tool that helps researchers analyze a given implementation and understand the reasons why it may perform better or worse than some other implementation.
%As an example, for a fixed algorithm and implementation, a graph can be rearranged such that the actual amount of work performed in counting triangles changes, without any change in the number of edges.
%Hence, using a metric such as Edges per Second, researchers may attribute speedup in an implementation due to increased throughput, rather than a reduction in overall work.
%Therefore, in place of Edges per Second, we suggest that researchers adopt an alternate metric: Effective Matches Checked per Second (EMCs).

%We first explain Matches Checked per Second (MCs) in terms of a naive kernel for Triangle Counting. 
%Then, we introduce a more nuanced variant of the metric appropriate for TC algorithms that may in fact do more work: effective Matches Checked Per Second (EMCs).
%For the naive approach, effective Matches Checked Per Second is the same as Matches Checked per Second.
%We demonstrate the comparison of the naive scalar algorithm against a straightforward SIMD approach for Triangle Counting, showing that in microbenchmarks the SIMD kernel has an overall speedup of XX times the EMCs compared to the naive scalar kernel. 
%On the suite of GraphChallenge graphs, a hybrid Triangle Count implementation incorporating the scalar and SIMD kernels reaches an average performance of XX EMCs, while the scalar kernel acheives an average of XX EMCs.



%In Section~\ref{section:metric}, we introduce our proposal for a metric that better describes the performance of a triangle counting implementation. 
%We relate the metric to the work performed from a graph-algorithmic perspective, and then elaborate on what the metric means from a hardware perspective.
%In Section~\ref{section:sorting_study}, we demonstrate the explanatory utility of our metric on a common graph pre-processing strategy.
%Section~\ref{section:scalar_and_SIMD}, we discuss the basic approach in Algorithm~\ref{alg:scalar_inter} and compare it to a SIMD approach for triangle counting. 
%We discuss the performance attained by several recent GraphChallenge submissions for triangle counting in Section~\ref{section:existing_approaches}.
%Finally, we conclude and note opportunities for future work in Section~\ref{section:conclusion}.

==> TC_Perf cam ready plus ieee copyright/intro_draft_MB.tex <==
Exact Triangle Counting is a commonly used benchmark graph application, present both in the Graph Analytics Benchmark suite as well as an established subproblem for several years in the GraphChallenge competition.
Since the inclusion of Triangle Counting (TC) in GraphChallenge, performance for TC has increased manyfold.
Throughout years of performance advances, TC has lacked a meaningful and objective metric that describes the work being performed and can be used to compare implementations across platforms, graphs, and architectures.
Instead, performance is reported in terms of Edges Per Second or some similar variant, which is in essence the runtime to process the graph normalized by an approximation of its size in number of edges.
However, this figure of merit has little to do with the work being performed at the core of TC: two graphs of similar number of edges may have very different topologies, leading to very different runtimes.

The lack of an objective metric for the performance of Triangle Counting makes it difficult to properly analyze a given implementation and understand the reasons why it may perform better or worse than some other implementation or why performance may suffer on one graph compared to another.
Further, for a fixed algorithm, implementation, and graph, a single graph can be rearranged such that the actual amount of work performed in counting triangles changes without any change in the number of edges.
Using a misleading metric such as Edges per Second, researchers may attribute speedup in an implementation due to increased throughput, rather than a reduction in overall work, as one possible pitfall.
Therefore, in place of Edges per Second, we suggest that researchers adopt an alternate metric: Matches Checked per Second (MCs).


We first explain the origin of this metric, Matches Checked per Second (MCs), in terms of a naive kernel for Triangle Counting. 
Then, we introduce a more nuanced variant of the metric appropriate for TC algorithms that may in fact do more work: 
effective Matches Checked Per Second (EMCs).
For the naive approach, effective Matches Checked Per Second is the same as Matches Checked per Second.
We demonstrate the comparison of the naive scalar algorithm against a straightforward SIMD approach for Triangle Counting, showing that in microbenchmarks the SIMD kernel has an overall speedup of XX times the EMCs compared to the 
naive scalar kernel. 
On the suite of GraphChallenge graphs, a hybrid Triangle Count implementation incorporating the scalar and SIMD kernels reaches an average performance of XX EMCs, while the scalar kernel acheives an average of XX EMCs.



==> TC_Perf cam ready plus ieee copyright/metric.tex <==
%A challenging aspect of determining a performance metric for TC, even for a fixed architecture, is that the graph itself being processed affects how execution of triangle counting's primitive operations proceed. 
%To aid in the search for an objective performance metric for triangle counting, 

For the sake of completeness, we begin with a brief description of triangle count and commonly used approaches for computing the number of triangles in a graph. We then derive a plausible performance metric for the triangle count operation: match checks.
%stating a few basic assumptions, and then discuss a scalar set intersection kernel within TC.

\subsection{Triangle Counting}
Triangle counting, as its name suggests, counts the number of triangles in a undirected graph $G$. This graph can be represented by its adjacency matrix which is a symmetric sparse matrix.  For the purposes of this paper, we assume that only the lower-triangular portion of the adjacency matrix is stored.

Processing only the lower-triangular (or upper) part of the adjacency matrix allows one to count each triangle exactly once. This approach is common in many implementations~\cite{lee_family_2017, azad_parallel_2015, voegele_parallel_2017}.
Elements in this part of the matrix correspond to edges leading from one vertex to a neighbor with lower vertex ID. This portion of each vertex's neighborhood is referred to as the lower neighborhood, denoted as $N_l(v)$ for vertex $v$.
%For the purpose of triangle counting, we are neither concerned with the direction of edges nor their weight; 
%hence, we consider any graph to be processed to have symmetric, unweighted edges.
%Generally, this means that for every edge $(u,v)$ in the set of edges $E$,
%the reversed edge, $(v,u)$, is also present.
%The connectivity of the graph can this be represented as an upper- or lower-triangular sparse adjacency matrix.%, of which only the 
%is needed to describe the graph's connectivity.

%The symmetry of the graph allows algorithms to avoid examining all edges in searching for triangles.
%For example, the approaches of \cite{} all take advantage of the graph symmetry by 
%only processing half of the adjacency matrix.% or constraining which edge directions may be considered in triangles. 
%For the purposes of this paper, we follow the convention of processing the lower-triangular portion of the adjacency matrix.


%Is this really necessary?

%\subsection{Graph Format}
%In our discussion of the triangle counting algorithm, we make several assumptions on the format of the graph.
%First, we assume that the graph is stored in compressed sparse row (CSR) format, as two arrays, in memory.
%Edges are represented by vertex IDs in the neighborhoods of each vertex, and these IDs are sorted in increasing order within each neighborhood.
%As the graph is symmetric this CSR representation only stores the lower-numbered part of each vertex's neighborhood - that which contains lower numbered neighbors than it.

\subsection {Exact triangle count with wedges and intersections}

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/wedge_check_vertex_compare_set_intersect.pdf}
    \caption{Diagram of connected vertices $v$ and $u$. To count triangles, their lower neighborhoods are intersected, with $u$ subtracted from $N_l(v)$. $\Delta$ is the triangle count.}
    \label{fig:wedge_match_check}
\end{figure}

In general, there are two approaches to counting the number of triangles in a graph. 
The first method is the wedge-check method, where given a wedge (i.e. three vertices connected with two edges), a check is performed to test if there exists an edge that closes the wedge into a triangle. The second approach, based on set-intersection, identifies if there exists a common vertex in the neighborhood of the two vertices of an edge.

% The two approaches are illustrated by Fig.~\ref{fig:wedge_match_check}.
% Either a wedge connecting $u$ and $v$ is found (e.g. $(v,w_0,u)$ or $(v,w_1,u)$), and the check for an edge connecting $v$ and $u$ succeeds, locating 
We demonstrate the equivalence of the two approaches using Fig.~\ref{fig:wedge_match_check}.
In the following discussion, $v>u$ for both approaches.
In the wedge-check method, the wedges between each pair of vertices $v$, $u$ are found by way of the shared neighbors (e.g. the vertices labeled $x_0/y_0$ and $x_1/y_2$) between their lower neighborhoods ($N_l(v), N_l(u)$). 
The existence of the triangle is then confirmed by checking for the edge directly connecting $v$ to $u$.
In the set-intersection approach, for the endpoints of an existing edge $(v, u)$, their lower neighborhoods are intersected to find shared neighbors (again, $x_0/y_0$ and $x_1/y_2$ in the diagram). Because the intersection is only performed given that edge $(v, u)$ exists, each shared neighbor found in the intersection indicates a triangle.

In practice, work for the first approach is often pre-filtered by existing edges, fusing the two steps and making the two approaches equivalent.
These ways of describing triangle counting mechanics are also compatible with sparse-matrix based approaches. In particular, the work by Wolf et al. for miniTri specifically highlights a wedge-check approach based on a linear algebraic specification~\cite{wolf_task-based_2015}.

%Finding triangles from the lower-triangular adjacency matrix proceeds as follows.
%For each lower-neighbor of each vertex, an edge exists between the parent vertex and the lower-neighbor.
%Fig.~\ref{fig:wedge_match_check} labels the two vertices in this case as $v$ and its lower-neighbor $u$.
%Next, $v$ and $u$ may each have some additional neighbors in their lower-neighborhoods, $x_i$ and $y_j$ for example.
%In the case that some $x_i$ and $y_j$ turn out to be the same vertex, and not one of $v$ or $u$, a triangle has been found.

%Graphically, this can be seen as a comparison of the endpoints of two wedges that are already known to be partially overlapping: $(u, v, x_i)$ and $(v, u, y_j)$. Alternatively, this can be viewed as searching for wedges that connect vertices $u$ and $v$ through some vertex $w=x_i=y_j$, which closes a wedge with the existing edge from $v$ to $u$, forming a triangle.

From either perspective, the work of finding wedges that may close into triangles constitutes an intersection of $N_l(v)$ and $N_l(u)$.
Algorithm~\ref{alg:scalar_inter} illustrates the core operation in triangle counting by way of a naive approach for set intersection, commonly referred to as merge-based set intersection as in~\cite{inoue_faster_2014, DBLP:conf/icde/ZhangLSF20}.
 
\begin{algorithm}[tb]
\DontPrintSemicolon
\smaller
\KwIn{a1 and a2 initially give the start addresses of each set. a1\_nd and a2\_nd are the addresses just after the end of each set.}
\KwOut{$\Delta$ is the number of matches among both sets.}
\BlankLine
$\Delta \leftarrow 0$ \\
\While{a1 $<$ a1\_nd $\land$ a2 $<$ a2\_nd} {
      \If{*a1 == *a2} {
        a1 $\leftarrow$ a1 + 1\\
        a2 $\leftarrow$ a2 + 1\\
        $\Delta \leftarrow \Delta + 1$\\
      }
      \ElseIf {*a1 $>$ *a2} {
        a2 $\leftarrow$ a2 + 1\\
      }
      \Else {
        a1 $\leftarrow$ a1 + 1\\
      }
  }
  \Return{$\Delta$} \\
  \caption{Scalar merge-based set intersection kernel. Asterisk (*) before an address symbol indicates access to memory.}
  \label{alg:scalar_inter}
\end{algorithm}

\subsection {Expected work for Exact Triangle Count}
%\subsection{Deriving a Metric from Set Intersection}
%In the domain of graph algorithms, edges per second is often used as a figure of merit for any given graph application. 
%For triangle counting, this figure of merit, however, is neither portable between graphs, nor portable between hardware. 
%Between two graphs of the same number of edges and vertices, the manner in which graphs are connected may have a stark effect on runtime; although the numbers of edges may be identical, the achieved edges per second differ greatly.
%Edges per second clearly cannot give a sense of the performance potential achieved or why one graph may be harder to process than the other.

Given the previous discussion, the 
core operation in triangle counting can be viewed as finding the size of neighborhood set intersections. Given two neighborhoods of vertices, the first vertex in each of the two neighborhoods are compared (intersected).
%The direct-yet-efficient approach is to use scalar functional units, intersecting pairs of vertex IDs one at a time.
In the case of a match, the match is recorded and the next vertices in each neighborhood are compared. Otherwise, the next vertex in the neighborhood of the vertex with the smaller of the IDs is compared with the vertex with the larger ID. This process is repeated until all vertices in one or both neighborhoods have been checked. 
% An implementation of this algorithm is provided in  Algorithm~\ref{alg:scalar_inter}.

Notice that this work has to be performed even if there are no triangles in the graph since the absence of any triangle can only be ascertained after iterating through the neighborhoods.
This suggests that the number of match checks a graph requires better reflects the amount of work in triangle counting than the number of edges does. 
In addition, the number of match checks performed by triangle counting equals the number of iterations executed by the loop in Algorithm~\ref{alg:scalar_inter}.
From this point in the paper, we refer to such wedge or vertex comparisons as \emph{match checks or matches}.


%We observed that the innermost loop, or kernel, of Algorithm~\ref{alg:scalar_inter} performs set intersections between neighborhoods of two already connected vertices in the graph.
%Hence, the loop compares two \textit{wedges} formed by the pair of parent vertices and one of each of their neighbors.
%If the two neighbors are the same, then the wedges under consideration are in fact the same, and a triangle is counted.
%From this we conclude that the items of work performed in triangle counting are wedge match checks, or wedge comparisons, which may also be seen simply as vertex ID comparisons.
%Since the body of the innermost loop checks for matches, the number of wedge pairs that are compared for any given graph corresponds exactly to the number of iterations executed by the loop in .

\subsection{Match Checks in Hardware}
% In hardware, match checks can be accomplished in an number of ways.
% A match can be checked by comparison, followed by jumps to change control flow to the correct operations needed.
% This strategy is used in Algorithm~\ref{alg:scalar_inter} with a three-way branch to express the case of a match, and the two sub-cases when a match check returns false.
% Instead of branching, predicated instructions could alternatively be used following the comparison of the two vertex IDs. 
As a metric, match checks do not prescribe which instructions or implementation should be used, but generally indicate that some form of compare instruction followed by conditional updates are required for each match check. Possible implementations of 
Algorithm~\ref{alg:scalar_inter} include 1) a compare operation followed by branches, and 2) predicated instructions to avoid branches~\cite{DBLP:conf/icde/ZhangLSF20}.

However, knowing how match checks are mapped (either manually or by the compiler) to specific instructions or hardware components allows us to use match checks as a proxy for the amount of hardware resources required to compute the necessary amount of work. For example, mapping match checks to a compare instruction naturally limits the rate of match checks to the throughput of the compare (\texttt{CMP}) instruction on a given architecture.

%Nonetheless, the number of match checks that must be performed remains the same.
%In this way, match checks link a graph-algorithmic operation, comparing the endpoints of two wedges, to the conditional handling of a compare operation on two values.
% The metric of work that we specifically propose is the number of match checks that the example algorithm would perform. 

%\subsection{Canonical Number of Match Checks}
% Setting aside additional optimizations that may be able to skip intervals of values in one of the neighborhoods, 
%Algorithm~\ref{alg:scalar_inter} exhibits a well-defined number of matches to check.
%Owing to the ordering of the vertex neighborhoods, not every combination of wedges must be considered. 
%However, matches that fail to yield triangles cannot be entirely eliminated; checking them ahead of time to eliminate them would amount to doing triangle counting in the first place.
%Therefore, the metric of match checks processed, either per second or per cycle, is linked to the graph by way of this algorithm, giving the minimum number of match checks that must be processed to find all triangles in the graph.

%In the next section, we demonstrate the utility of matches as a metric of work and match check rate as a metric of performance. We show that the number of match checks correlates with runtime of triangle count, that the number of match checks for a graph is not fixed, and that the change in number of match checks for a relabeled graph also correlates with the changed runtime of while the number of edges remains constant. 

==> TC_Perf cam ready plus ieee copyright/real_world.tex <==
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{figures/scalar_simd_snap.pdf}
    \caption{Effective Matches per Second for the scalar approach and a multi-kernel SIMD approach. SIMD tends to have a higher match check rate than scalar, but not to the extent seen in the microbenchmarks.}
    \label{fig:scalar_vs_SIMD}
\end{figure*}

\subsection{Analysis of TC with Match Checks per Second}
From the insight that match checks are triangle counting's algorithmic units of work and considering the limitations of the scalar approach in processing them, we arrived at the SIMD approach benchmarked in the previous section.
The Effective Match Check rate accurately reflected the advantage of performing many potentially unnecessary compares over the original scalar implementation.
% Fig.~\ref{fig:scalar_vs_SIMD} presents a summary of performance in millions of effective match checks per second.
Using Effective Matches per Second, we now compare the scalar approach with a multi-kernel SIMD approach, similar to the one described for the microbenchmark, but for exact triangle counting. 
Fig.~\ref{fig:scalar_vs_SIMD} shows that the SIMD approach reaches a higher match check rate than the scalar approach, but not to the extent seen in the benchmarks. Taking into account the multi-case nature of the SIMD approach, this suggests that the performance benefits are realized only for some fraction of the set intersections.
These results also show that the metric used here, Effective Match Checks per Second, accurately portrays that some overheads in dealing with the graph and in having shorter set intersections than in the idealized microbenchmark reduce the performance impact of the SIMD approach.

% The performance numbers show that for most graphs, the metric of effective matches per second indeed reflects that SIMD performs better than the scalar approach. Of note, the metric also makes it clear that some graphs do not benefit from SIMD. Upon further inspection of the implementation, this can be verified in that NEED TO DO A QUICK TEST...

==> TC_Perf cam ready plus ieee copyright/sorting.tex <==
In this section, we demonstrate that match checks are an acceptable metric for work in triangle counting. %and that effective match check rate (per second, per cycle) is a more objective performance metric than edges per second.
%We do this by reviewing a few techniques used in triangle counting, including sort and use of alternate algorithms and hardware. We use graphs from the SNAP dataset \cite{snapnets} and GraphChallenge~\cite{samsi_static_2017}.

\begin{figure}
    \centering
    % \includegraphics[width=\linewidth]{figures/Number of Match Checks and Graph Runtime.pdf}
    % \caption{Number of match checks plotted against runtime in seconds for scalar merge-sort-based triangle counting. Increased number of match checks generally correspond to increased runtime.}
    \includegraphics[width=\linewidth]{figures/Number_of_Match_Checks_and_Edges_vs_Graph_Runtime.pdf}
    \caption{Number of match checks and edges plotted against runtime for scalar merge-sort-based triangle counting, for 3 graph orderings per graph. Increased number of match checks and edges both generally correspond to increased runtime. Match checks show a stronger fit to runtime ($r^2=0.94$) compared to raw number of edges ($r^2=0.884$).}
    \label{fig:runtime_and_checks}
    \vspace{-5mm}
\end{figure}

\subsection{Matches Reflecting Work in Triangle Count}
We validate the use of match checks as a metric of the work for triangle count in Fig.~\ref{fig:runtime_and_checks}.
Each point represents a graph from a real or synthetic graph in the Graph Challenge dataset, processed using a sequential merge-based triangle count implementation~\cite{samsi_static_2017, snapnets}.
The number of match checks per graph was obtained from a second non-timing run, shown in blue.
%as the number of times through the while loop of Algorithm~\ref{alg:scalar_inter}.
As expected, the runtime increases with increased number of match checks across the 93 graphs. Hence, match checks are a representative metric for the work in triangle counting. 
By contrast, we also show the number of edges in each graph in red in Fig.~\ref{fig:runtime_and_checks}. While there is clearly some correlation between the number of edges in a graph and the number of checks, it is a weaker one. 

% Comment from Mark: this statement (below) is less compelling when also showing EPs.
% An interesting observation is that despite having different sizes of graphs that fit into different layers in the memory hierarchy, the scatter plot in Figure~\ref{fig:runtime_and_checks} falls within a narrow band. 

\subsection{Matches Reflecting Implementation Innovation}
%At this point we have identified match checks as a unit of work and presented initial evidence that they accurately reflect work in triangle counting. However, we have not addressed the dynamic between this metric, the number of edges in a graph, and vertex labeling.

It has been observed in numerous works that graph reordering can improve triangle counting performance. 
Chiba and Nishizeki observed that processing vertices in decreasing order of degree enables better running-time bounds for triangle counting based on the graph's aboricity~\cite{chiba_arboricity_1985}.
Recent Graph Challenge implementations such as Bisson et al. attribute improvements in performance to more balanced threads on the GPU~\cite{bisson_update_2018}.
More generally for graph algorithms, Balaji et al. note improvements due to improved memory layout and access patterns~\cite{balaji_when_2018}.
Using the proposed matches-checked metric, we show that new insights can be gained into the need for sorting. 
%However, when viewing the work to be performed in triangle counting in terms of match checks, it becomes apparent that relabeling the vertices in a graph can have a profound effect on the number of matches that need to be performed, and at least in part, it is from this that a change in runtime comes.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/Speedup_vs_Change_in_Match_Checks_Due_to_Sort.png}
    \caption{Speedup over non-sorted graph plotted against the change in number of match checks performed for different graph sorts. Different markers represent sort orders. Different sort orders are necessary on different graphs to reduce match checks and execution time.}
    \label{fig:sort_matches}
    \vspace{-5mm}
\end{figure}

\noindent{\em Observation 1: Sorting changes the number of match checks performed.} Besides load-balancing, sorting in the appropriate fashion can significantly reduce the amount of work. 
Fig.~\ref{fig:sort_matches} shows the speedup of triangle counting against the decrease (below 1) or increase (above 1) in proportion of match checks over the unsorted original graph for sequential triangle count. The number of match checks is changed by relabeling vertices based on degree in decreasing order (blue) or increasing order (red). 
% We emphasize that the triangle counting implementation we use processes the lower-triangular portion of each vertex neighborhood - the neighboring vertices with ID less than the parent of the neighborhood itself.
%Because tests were performed with a single thread to exclude multi-threaded effects, 
%As the implementation is sequential, the changes in performance that we observe are due to the change in match checks performed along with possible changes to the memory locality of the graph.
% Generally, sorting the graph from largest to smallest degree \textsl{decreases} the number of match checks to be performed, while sorting in the reverse direction \textit{increases} the number of checks.
For most graphs, we observe that sorting changes the number of match checks performed, and thus a corresponding change in execution time is observed.

{\em Observation 2: Different label orders are required for different graphs.}
While sorting vertices by decreasing vertex degree often leads to lower execution time, a number of graphs benefit from sorting in the reversed order. This is demonstrated in Fig.~\ref{fig:sort_matches} when certain red triangular markers are in the bottom right quadrant, while a small number of blue circular markers are in the top left quadrant.  This suggests that a possible area of future research into heuristics that determine the appropriate sort order or alternative labeling for a given graph.


%There are exceptions: roadNet-CA and some oregon1 networks see reduced numbers of match checks while taking slightly longer to run. 
%ca-GrQc and ca-HepPh speed up by 1.3x but have 30\% more match checks.

%However, most of the graphs in this collection still fit the general trend: more match tests results in a longer runtime, and fewer match tests result in lower runtime.
%Using match checks as a metric here reveals that much of the speedup attributed to sorting, in either direction, comes from a change in the amount of work performed, and largely explains why sorting in one way for all graphs is not always faster.

% We note that the number of triangles and edges in each graph do not change while often the runtimes change significantly.
% This exemplifies the pitfall of using edges per second to measure performance: such a metric suggests that the number of edges give an accurate picture of the amount of work in triangle counting.
% In contrast, this experiment demonstrates the utility of match checks as a unit of work in triangle counting.


% Therefore, match checks per second should be considered for use as a performance metric.



==> conclusion_draft.tex <==
In summary, this work seeks to address the limitations of using Edges Per Second as a performance metric for Exact Triangle Counting (TC).
As an alternative, we proposed a basic metric based on examination of a naive scalar kernel for TC: Matche Checks per Second (MCs).
We motivated the metric by its ability to better describe the amount of work performed in a triangle counting implementation based on identifying matching pairs of vertex IDs that complete a found triangle.
By using graph reordering, a common preprocessing step, we illustrated the descriptive value of the metric:
in the oregon1\_010519 of the GraphChallenge collection the match checks to be performed decreased by 97 percent, leading to a 19.9x speedup for the same scalar implementation;
when sorting in the reverse order increased the number of checks performed in p2p-Gnutella09 by 30 percent, processing the graph took 4.2 times longer.
Using a work-inefficient SIMD implementation as an example, we showed that the metric can apply to more complex approaches by way of measuring performance in terms of Effective Match Checks per Second (EMCs).

Effective Match Checks per Second as a metric is intended to be a useful tool in focusing researchers' reasoning about Exact Triangle Counting implementations and how those implementations perform on various graphs and hardware.
Using EMCs as a starting point, we hope to bring the community's understanding of TC one step closer to being able to reason about implementation performance in terms of hardware performance peaks.

==> intro_draft_MB.tex <==
Exact Triangle Counting is a commonly used benchmark graph application, present both in the Graph Analytics Benchmark suite as well as an established subproblem for several years in the GraphChallenge competition.
Since the inclusion of Triangle Counting (TC) in GraphChallenge, performance for TC has increased manyfold.
Throughout years of performance advances, TC has lacked a meaningful and objective metric that describes the work being performed and can be used to compare implementations across platforms, graphs, and architectures.
Instead, performance is reported in terms of Edges Per Second or some similar variant, which is in essence the runtime to process the graph normalized by an approximation of its size in number of edges.
However, this figure of merit has little to do with the work being performed at the core of TC: two graphs of similar number of edges may have very different topologies, leading to very different runtimes.

The lack of an objective metric for the performance of Triangle Counting makes it difficult to properly analyze a given implementation and understand the reasons why it may perform better or worse than some other implementation or why performance may suffer on one graph compared to another.
Further, for a fixed algorithm, implementation, and graph, a single graph can be rearranged such that the actual amount of work performed in counting triangles changes without any change in the number of edges.
Using a misleading metric such as Edges per Second, researchers may attribute speedup in an implementation due to increased throughput, rather than a reduction in overall work, as one possible pitfall.
Therefore, in place of Edges per Second, we suggest that researchers adopt an alternate metric: Matches Checked per Second (MCs).


We first explain the origin of this metric, Matches Checked per Second (MCs), in terms of a naive kernel for Triangle Counting. 
Then, we introduce a more nuanced variant of the metric appropriate for TC algorithms that may in fact do more work: 
effective Matches Checked Per Second (EMCs).
For the naive approach, effective Matches Checked Per Second is the same as Matches Checked per Second.
We demonstrate the comparison of the naive scalar algorithm against a straightforward SIMD approach for Triangle Counting, showing that in microbenchmarks the SIMD kernel has an overall speedup of XX times the EMCs compared to the 
naive scalar kernel. 
On the suite of GraphChallenge graphs, a hybrid Triangle Count implementation incorporating the scalar and SIMD kernels reaches an average performance of XX EMCs, while the scalar kernel acheives an average of XX EMCs.



==> real_world.tex <==
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{figures/scalar_simd_snap.pdf}
    \caption{Effective Matches per Second for the scalar approach and a multi-kernel SIMD approach. SIMD tends to have a higher match check rate than scalar, but not to the extent seen in the microbenchmarks.}
    \label{fig:scalar_vs_SIMD}
\end{figure*}

\subsection{Analysis of TC with Match Checks per Second}
From the insight that match checks are triangle counting's algorithmic units of work and considering the limitations of the scalar approach in processing them, we arrived at the SIMD approach benchmarked in the previous section.
The Effective Match Check rate accurately reflected the advantage of performing many potentially unnecessary compares over the original scalar implementation.
% Fig.~\ref{fig:scalar_vs_SIMD} presents a summary of performance in millions of effective match checks per second.
Using Effective Matches per Second, we now compare the scalar approach with a multi-kernel SIMD approach, similar to the one described for the microbenchmark, but for exact triangle counting. 
Fig.~\ref{fig:scalar_vs_SIMD} shows that the SIMD approach reaches a higher match check rate than the scalar approach, but not to the extent seen in the benchmarks. Taking into account the multi-case nature of the SIMD approach, this suggests that the performance benefits are realized only for some fraction of the set intersections.
These results also show that the metric used here, Effective Match Checks per Second, accurately portrays that some overheads in dealing with the graph and in having shorter set intersections than in the idealized microbenchmark reduce the performance impact of the SIMD approach.

% The performance numbers show that for most graphs, the metric of effective matches per second indeed reflects that SIMD performs better than the scalar approach. Of note, the metric also makes it clear that some graphs do not benefit from SIMD. Upon further inspection of the implementation, this can be verified in that NEED TO DO A QUICK TEST...
